Feature Engineering and Classification Models for Partial Discharge in Power Transformers

To ensure reliability, power transformers are monitored for partial discharge (PD) events, which are symptoms of transformer failure. Since failures can have catastrophic cascading consequences, it is critical to preempt them as early as possible. Our goal is to classify PDs as corona, floating, particle, or void, to gain an understanding of the failure location. Using phase resolved PD signal data, we create a small set of features, which can be used to classify PDs with high accuracy. This set of features consists of the total magnitude, the maximum magnitude, and the length of the longest empty band. These features represent the entire signal and not just a single phase, so the feature set has a fixed size and is easily comprehensible. With both Random Forest and SVM classification methods, we attain a 99% classification accuracy, which is significantly higher than classification using phase based feature sets such as phase magnitude. Furthermore, we develop a stacking ensemble to combine several classification models, resulting in a superior model that outperforms existing methods in both accuracy and variance.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex

###############################################################################
# the main latex file is ascem.tex in this directory
MAIN = pd_classification_paper

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex}
BIBFILES = ${wildcard *.bib}
#FIGS = figs/${wildcard}/${wildcard *.png}
#FIGS = figures/${wildcard *.pdf}
FIGS = 

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

# RM used in many places, make sure it is defined
ifndef RM
RM=/bin/rm
endif

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex $(MAIN); ${LATEX} $(MAIN); fi;
	@while grep 'Rerun to get ' $(MAIN).log; \
        do ${LATEX} $(MAIN); \
        done
report.pdf report.log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} report
	@if [ `fgrep undefined report.log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex report; ${LATEX} report; fi;
	@if [ `fgrep undefined report.log | fgrep Citation - | wc -l` -gt 0 ]; then \
	bibtex report; ${LATEX} report; fi;
	@while grep 'Rerun to get ' report.log; \
        do ${LATEX} report; \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	bibtex $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . -name '*.aux' -o -name '*.log' -o -name '*.bbl' -o -name '*.blg' \
		-o -name '*.toc' -o -name '*.out' -o -name '*.ent' | xargs $(RM)

realclean: clean
	$(RM) $(MAIN).pdf $(MAIN).ps


==> discussion.tex <==
\label{sec:discussion}
The accuracy metric we used to determine the best model was \textbf{recall},
which is the number of each class that is classified as such.
For one PD type, this is calculated by 
\begin{align*}
\text{recall} = \frac{\text{number of predicted and actual corona PDs}}{\text{number of actual corona PDs}}
\end{align*}
To better understand the misclassifications, we also look at the \textbf{precision}, calculated by
\begin{align*}
\text{precision} = \frac{\text{number of predicted and actual corona PDs}}{\text{number of predicted corona PDs}}
\end{align*}
For \textit{floating} PDs, the recall is higher than precision, 
and it is the opposite for \textit{void} PDs as shown in Table~\ref{tab:precision_recall}.
For \textit{corona} and \textit{particle} PDs, the precision and recall are both about one.
This indicates that \textit{void} PDs are being misclassified as \textit{floating} PDs.
However, the difference between precision and recall in our results is very small as both values are close to one.
These values are also obtained by averaging over 100 experiments,
so only a few models of the 100 models we train have a few misclassified samples.

\begin{table}[tb]
\caption{Precision and Recall of each PD Type}
\label{tab:precision_recall}
\centering
\begin{tabular}{ | c | c | c | }
  \hline
  PD Type & Recall & Precision \\ \hline
  Corona & 0.998 & 1 \\ \hline
  Floating & 1 & 0.991 \\ \hline
  Particle & 0.999 & 1 \\ \hline
  Void & 0.988 & 1 \\ \hline
  \end{tabular}
\end{table}

Based on our meta-features, there were several outlier points.
We originally set the significance threshold for the empty band at 50\% of the maximum magnitude.
However, this resulted in several outliers, as shown in Figure~\ref{fig:features_empty_max_mag_50_outliers}.
The two outliers caused by the length of the longest empty band are a \textit{particle} PD and a \textit{void} PD.
In the case of the \textit{particle} PD in Figure~\ref{fig:2007-09-06-19-43-31_heatmap},
there a a few high magnitude points, which cause most points to become insignificant.
Similarly, in the \textit{void} PD case in Figure~\ref{fig:2006-06-13-18-00-44_heatmap},
a small band of high magnitude points makes the rest of the points insignificant.

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/features_empty_max_mag_50_outliers}
\caption{Outliers using 50\% Significance Threshold}
\label{fig:features_empty_max_mag_50_outliers}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/2007-09-06-19-43-31_heatmap}
\caption{Particle PD Outlier}
\label{fig:2007-09-06-19-43-31_heatmap}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/2006-06-13-18-00-44_heatmap}
\caption{Void PD Outlier}
\label{fig:2006-06-13-18-00-44_heatmap}
\end{figure}

By reducing the significance threshold to 40\%, we eliminate these outliers, 
leaving only the \textit{corona} outlier shown in Figure~\ref{fig:features_empty_max_mag_40_outliers}.
This outlier is just a high magnitude case as shown in Figure~\ref{fig:2007-09-06-17-10-06_heatmap}.
It has a significantly higher maximum magnitude and a wider band than all other \textit{corona} samples.
Since this outlier can still be separated from the \textit{void} PDs by the total magnitude, 
we do not take any further action to address it.
Lowering the significance threshold further impedes the ability to distinguish noise points.

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/features_empty_max_mag_40_outliers}
\caption{Outliers using 40\% Significance Threshold}
\label{fig:features_empty_max_mag_40_outliers}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/2007-09-06-17-10-06_heatmap}
\caption{Corona PD Outlier}
\label{fig:2007-09-06-17-10-06_heatmap}
\end{figure}

The last case of interesting sample points is the \textit{void} PDs with higher maximum magnitude.
An example of this is illustrated in Figure~\ref{fig:2007-10-17-12-08-26_heatmap}.
A few high magnitude points in this sample raises the maximum magnitude.
Unfortunately, there are enough high magnitude points 
such that it is not captured by the maximum magnitude averaging to prevent high magnitude outlier points.
Again, since these outliers can be separated from the \textit{floating} PDs by total magnitude,
we do not examine these outliers further.

\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{figures/2007-10-17-12-08-26_heatmap}
\caption{Void PD Maximum Magnitude Outlier}
\label{fig:2007-10-17-12-08-26_heatmap}
\end{figure}

Based on this examination of outliers, we notice that several of the PD types can be sub-classified.
For example there are three types of \textit{corona} PDs as shown in Figure~\ref{fig:corona_subtypes}
and two types of \textit{floating} PDs as shown in Figure~\ref{fig:floating_subtypes}.
The corona PDs are divided by the phase at which the signal occurs, 
either at high phases (Figure~\ref{fig:2006-06-13-14-15-29_heatmap}) 
or low phases (Figure~\ref{fig:2006-06-07-15-10-28_heatmap}) 
or both (Figure~\ref{fig:2006-06-07-15-11-06_heatmap}).
The distinction between the two phase \textit{coronas} and the one phase \textit{coronas}
is clear based on the two clusters based on the length of the longest empty band.
Similarly, \textit{floating} PDs have straight bands (Figure~\ref{fig:2006-06-07-17-10-51_heatmap}) 
and curved bands (Figure~\ref{fig:2006-06-07-18-00-37_heatmap}).
While there are different subtypes of the PDs, this subclassification is beyond the scope of this project,
since we are only looking at the four primary classifications - \textit{corona}, \textit{floating}, \textit{particle}, and \textit{void},
but may be addressed in future work by adding additional features and labels.

\begin{figure}
\begin{subfigure}[tb]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figures/2006-06-07-15-10-28_heatmap}
\caption{Corona PD - Low Phase}
\label{fig:2006-06-07-15-10-28_heatmap}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}[tb]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figures/2006-06-13-14-15-29_heatmap}
\caption{Corona PD - High Phase}
\label{fig:2006-06-13-14-15-29_heatmap}
\end{subfigure}

\begin{subfigure}[tb]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figures/2006-06-07-15-11-06_heatmap}
\caption{Corona PD - Two Phase}
\label{fig:2006-06-07-15-11-06_heatmap}
\end{subfigure}
\caption{Corona PD Subtypes}
\label{fig:corona_subtypes}
\end{figure}

\begin{figure}
\begin{subfigure}[tb]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figures/2006-06-07-17-10-51_heatmap}
\caption{Floating PD - Straight}
\label{fig:2006-06-07-17-10-51_heatmap}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}[tb]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figures/2006-06-07-18-00-37_heatmap}
\caption{Floating PD - Curved}
\label{fig:2006-06-07-18-00-37_heatmap}
\end{subfigure}
\caption{Floating PD Subtypes}
\label{fig:floating_subtypes}
\end{figure}

